Structure-Aware Transformer for Graph Representation Learning

The Transformer architecture has gained growing attention in graph representation learning recently, as it naturally overcomes several limitations of graph neural networks (GNNs) by avoiding their strict structural inductive biases and instead only encoding the graph structure via positional encoding. Here, we show that the node representations generated by the Transformer with positional encoding do not necessarily capture structural similarity between them. To address this issue, we propose the Structure-Aware Transformer, a class of simple and flexible graph Transformers built upon a new self-attention mechanism. This new self-attention incorporates structural information into the original self-attention by extracting a subgraph representation rooted at each node before computing the attention. We propose several methods for automatically generating the subgraph representation and show theoretically that the resulting representations are at least as expressive as the subgraph representations. Empirically, our method achieves state-of-the-art performance on five graph prediction benchmarks. Our structure-aware framework can leverage any existing GNN to extract the subgraph representation, and we show that it systematically improves performance relative to the base GNN model, successfully combining the advantages of GNNs and Transformers. Our code is available at https://github.com/BorgwardtLab/SAT.

==> graveyard.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Comparison to GNN Sparse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[t]
  \caption{Comparison of a base GNN and the augmented version with SAT.}
  \label{tab:comparison_to_sparse_GNNs}
  \centering
    \begin{small}
    \setlength{\tabcolsep}{0.50em}
      \begin{sc}
        %\resizebox{\textwidth}{!}{%
          \begin{tabular}{lccccc}
            \toprule
            {}&\multicolumn{2}{c}{\textbf{ZINC}}&\multicolumn{1}{c}{\textbf{CLUSTER}} &\multicolumn{1}{c}{\textbf{PATTERN}}&\multicolumn{1}{c}{\textbf{MOLPPA}}   \vspace{0.5em} \\
            Method & Edge weights & No edge weights & All & All & All \\
            \midrule
            GCN & N/A & 0.367 $\pm$ 0.011 &  68.498 $\pm$ 0.976 & 71.892 $\pm$ 0.334 \\
            GCN + SAT & N/A & 0.1767 $\pm$ 0.0038 & 77.247$\pm$0.094 & 86.749$\pm$0.065 \\
            GCN + SAT + KHOP & N/A & 0.1814 $\pm$ 0.0024 & & 86.816$\pm$0.028 \\
            \midrule
            GIN/GINE & & 0.387 $\pm$ 0.015 & 64.716 $\pm$ 1.553 & 85.590 $\pm$ 0.011 \\
            GIN/GINE + SAT & 0.1218 $\pm$ 0.0073 & 0.1663 $\pm$ 0.0009 & 77.255$\pm$0.085 & 86.759$\pm$0.022 \\
            GIN/GINE + SAT + KHOP & & 0.1621 $\pm$ 0.0099 & & 86.746$\pm$0.014 \\
            \midrule
            GraphSAGE & N/A & 0.398 $\pm$ 0.002 &  63.844 $\pm$ 0.110 & 50.516 $\pm$ 0.001 \\
            GraphSAGE + SAT & N/A & 0.1659 $\pm$ 0.0035 & 77.592$\pm$0.074 & 86.818$\pm$0.043 \\
            GraphSAGE + SAT + KHOP & N/A & 0.1683 $\pm$ 0.0054 & & 86.838$\pm$0.010 \\
            \midrule
            MPNN \\
            MPNN + SAT & 0.1176 $\pm$ 0.0057 & 0.1587 $\pm$ 0.0062 & \\
            MPNN + SAT + kHop & 0.0981 $\pm$ 0.0049 & 0.1385 $\pm$ 0.0027 \\
            \midrule
            PNA & 0.188 $\pm$ 0.004 & 0.320 $\pm$ 0.032 & N/A & N/A & N/A \\
            PNA + SAT & 0.1049 $\pm$ 0.0068 & 0.1465 $\pm$ 0.0043 & 77.751$\pm$0.121 & 86.865$\pm$0.043 \\
            PNA + SAT + kHop & 0.0935 $\pm$ 0.0082 & 0.1307 $\pm$ 0.0022 \\
            \bottomrule
        \end{tabular}
        %}
      \end{sc}
    \end{small}
\end{table*}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Comparison to SOTA Transformers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[tbp]
  \caption{Comparison of SAT to SOTA methods on graph regression and classification tasks. For ZINC, the metric is MAE, for CLUSTER and PATTERN, it is classification accuracy. For ZINC, the results use edge weights where applicable, else, the results without edge weights are reported.}
  \label{tab:comparison_to_SOTA}
  \centering
    \begin{small}
    \setlength{\tabcolsep}{0.50em}
      \begin{sc}
        %\resizebox{\textwidth}{!}{%
          \begin{tabular}{lccccc}
            \toprule
            {}&\multicolumn{2}{c}{\textbf{ZINC}}&\multicolumn{1}{c}{\textbf{CLUSTER}} &\multicolumn{1}{c}{\textbf{PATTERN}}&\multicolumn{1}{c}{\textbf{MOLPPA}}   \vspace{0.5em} \\
            Method & Edge weights & No edge weights & All & All & All \\
            \midrule
            GIN & - & 0.387$\pm$0.015 & 64.716$\pm$1.553 & 85.590$\pm$0.011 & 0.704$\pm$0.011 \\
            PNA & 0.188$\pm$0.004 & 0.320$\pm$0.032 & - & 86.567$\pm$0.075 \\
            GAT & - & 0.384$\pm$0.007 & 70.587$\pm$0.447 &  78.271$\pm$0.186 \\
            \midrule
            %
            SAN & 0.139$\pm$0.006 & - & 76.691$\pm$0.650 & 86.581$\pm$0.037 \\
            Graph Transformer & 0.226$\pm$0.014 & & 73.169$\pm$0.622 &  84.808$\pm$0.068 \\
            % GraphTrans \\
            Graphormer & 0.122$\pm$0.006 & - & - & - \\
            
            \midrule
            %
            GNN-SAT & 0.105$\pm$0.007 & 0.147$\pm$0.004 & 77.751$\pm$0.121 & 86.865$\pm$0.043 & 0.731$\pm$0.008 \\
            kHop-GNN-SAT & \textbf{0.092$\pm$0.007} & \textbf{0.133$\pm$0.001} \\
            \bottomrule
        \end{tabular}
        %}
      \end{sc}
    \end{small}
\end{table*}

\begin{comment}
        \resizebox{0.4\textwidth}{!}{%
          \begin{tabular}{lcccc}
                \toprule
                 \multicolumn{5}{c}{\textbf{ZINC, w/ edge weights}} \\
                 & GCN & GINE & GraphSAGE & PNA \\
                 \midrule
                 Base GNN & N/A & & N/A & 0.188$\pm$0.004\\
                 \midrule
                 k-subtree SAT & N/A & 0.115$\pm$0.005 & N/A & 0.102$\pm$0.005 \\
                 k-subgraph SAT & N/A & \textbf{0.095$\pm$0.002} & N/A & \textbf{0.094$\pm$0.008} \\
                 \bottomrule
          \end{tabular}
          }
          \hspace{4.5em}
          \vspace{1em}
          \resizebox{0.48\textwidth}{!}{%
          \begin{tabular}{lcccc}
                \toprule
                \multicolumn{5}{c}{\textbf{ZINC, w/o edge weights}} \\
                 & GCN & GIN & GraphSAGE & PNA \\
                 \midrule
                 Base GNN & 0.367$\pm$0.011 & 0.387$\pm$0.015 & 0.398$\pm$0.002 & 0.320$\pm$0.032 \\
                 \midrule
                 k-subtree SAT & 0.174$\pm$0.009 & 0.166$\pm$0.007 & \textbf{0.164$\pm$0.004} & 0.147$\pm$0.001 \\
                 k-subgraph SAT & 0.184$\pm$0.002 & \textbf{0.162$\pm$0.013} & \textbf{0.168$\pm$0.005} & \textbf{0.131$\pm$0.002} \\
                 \bottomrule
          \end{tabular}
          }
          
          \resizebox{.48\textwidth}{!}{%
          \begin{tabular}{lcccc}
                \toprule
                \multicolumn{5}{c}{\textbf{CLUSTER}} \\
                 & GCN & GIN & GraphSAGE & PNA \\
                 \midrule
                 Base GNN & 68.498$\pm$0.976 &  64.716$\pm$1.553 & 63.844$\pm$0.110 & 0.320$\pm$0.032 \\
                 \midrule
                 k-subtree SAT & 77.247$\pm$0.094  & 77.255$\pm$0.085 & 77.592$\pm$0.074  & 77.751$\pm$0.121 \\
                 k-subgraph SAT & \textbf{77.682$\pm$0.098} & \textbf{77.502$\pm$0.282} & \textbf{77.657$\pm$0.185} & 77.856$\pm$0.104  \\
                 \bottomrule
          \end{tabular}
          }
          \hspace{1em}
          \resizebox{0.48\textwidth}{!}{%
          \begin{tabular}{lcccc}
                \toprule
                \multicolumn{5}{c}{\textbf{PATTERN}} \\
                 & GCN & GIN & GraphSAGE & PNA \\
                 \midrule
                 Base GNN &  71.892$\pm$0.334 & 85.590$\pm$0.011 & 50.516$\pm$0.001  & 86.567$\pm$0.075 \\
                 \midrule
                 k-subtree SAT & 86.749$\pm$0.065 & \textbf{86.759$\pm$0.022} & 86.818$\pm$0.043 & 86.865$\pm$0.043  \\
                 k-subgraph SAT & \textbf{86.816$\pm$0.028} & 86.746$\pm$0.014 & \textbf{86.838$\pm$0.010} &  \\
                 \bottomrule
          \end{tabular}
          }
          \end{comment}

==> tables/pos_enc_table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% RW Positional Encoding Ablation Study
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[h!]
  \caption{Test MAE with and without the absolute random walk positional encoding on the ZINC dataset.}
  \label{tab:positional_encoding}
  \centering
    \begin{small}
    \setlength{\tabcolsep}{0.50em}
      \begin{sc}
        %\resizebox{\textwidth}{!}{%
          \begin{tabular}{lcc}
            \toprule
            & k-subtree SAT & k-subgraph SAT \\ 
            \midrule
            No abs. p.e.  & 0.177$\pm$0.007 & 0.097$\pm$0.003\\
            LAP abs. p.e. & 0.149$\pm$0.016 & \textbf{0.091$\pm$0.004} \\
            RW abs. p.e & \textbf{0.102$\pm$0.005} & 0.094$\pm$0.008\\
            
            \bottomrule
        \end{tabular}
        %}
      \end{sc}
    \end{small}
\end{table}

==> tables/readout_comparison.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% READOUT comparison
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[h!]
  \caption{Test MAE using different readout methods on ZINC.}
  \label{tab:readout}
  \centering
  \resizebox{\columnwidth}{!}{
    \begin{small}
    % \setlength{\tabcolsep}{0.50em}
      \begin{sc}
        %\resizebox{\textwidth}{!}{%
          \begin{tabular}{lccc}
            \toprule
            & Mean & Sum & Cls \\ 
            \midrule
            k-subtree SAT & 0.102$\pm$0.005 & 0.102$\pm$0.003 & \textbf{0.098$\pm$0.008} \\
            k-subgraph SAT & 0.094$\pm$0.008 & \textbf{0.089$\pm$0.002} & 0.093$\pm$0.009 \\
            \bottomrule
        \end{tabular}
        %}
      \end{sc}
    \end{small}
    }
\end{table}
